Was Javert right to be suspicious? Marginal Treatment Effects with Duration Outcomes

We identify the distributional and quantile marginal treatment effect functions when the outcome is right-censored. Our method requires a conditionally exogenous instrument and random censoring. We propose asymptotically consistent semi-parametric estimators and valid inferential procedures for the target functions. To illustrate, we evaluate the effect of alternative sentences (fines and community service vs. no punishment) on recidivism in Brazil. Our results highlight substantial treatment effect heterogeneity: we find that people whom most judges would punish take longer to recidivate, while people who would be punished only by strict judges recidivate at an earlier date than if they were not punished.

==> Preambles/header.tex <==
% Typesetting
\usepackage{changepage}
\newcommand\tab[1][1cm]{\hspace*{#1}}

    \usepackage[dvipsnames]{xcolor}
    \usepackage[T1]{fontenc}
	\usepackage[utf8]{inputenc}
	\usepackage[english]{babel}
    \usepackage{indentfirst}
    \usepackage{arydshln}

\usepackage[normalem]{ulem}
	\usepackage{amsfonts}
	\usepackage{amssymb}
	\usepackage{enumitem}
	    \usepackage{amsmath}
	\usepackage{adjustbox}
	%\usepackage{threeparttable}
\usepackage{adjustbox}
%\usepackage[normalem]{ulem}
	%\usepackage{enumerate}
	\usepackage{bbm}
	\usepackage{mathtools}
        \usepackage{caption}
        \usepackage{subcaption}
        \usepackage{relsize,exscale}
        \usepackage{multirow}
	\usepackage{booktabs}
	\usepackage[nodisplayskipstretch]{setspace}
	\usepackage{graphicx}
	\usepackage{fullpage}
	\def\labelitemi{--}
	\usepackage{soul}
	\usepackage{xspace}
	\usepackage{csquotes}
	\usepackage[margin = .9in]{geometry}
	\usepackage{placeins}
	\usepackage[footfont=normalsize,font=normalsize]{floatrow}
	\floatsetup[figure]{capposition=top}
	\floatsetup[table]{capposition=top}
	\usepackage{lscape}
	%\usepackage{longtable}
	\usepackage{mathabx}
    \usepackage{accents}
    \usepackage{float}
    \usepackage{pgffor}
    \usepackage{tikz}
    \usetikzlibrary{calc,intersections}
    \usepackage{xfrac}
    \usepackage{bigints}

% Bibliography
    % \usepackage[style=authoryear-comp,natbib=true,backend=biber]{biblatex}
    % \addbibresource{Bibliography.bib}
    % \usepackage{csquotes}
%	\usepackage{natbib}
	\usepackage[longnamesfirst]{natbib}
% 	\bibliographystyle{apalike}
	\bibliographystyle{aer}

 \definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
 \definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

% Links
	\usepackage{hyperref}

	\hypersetup{
    colorlinks=true,
    linkcolor=darkgreen,
    filecolor=magenta,
    urlcolor=darkgreen,
    citecolor = darkgreen
}
	\usepackage{cleveref}


% Theorems

    \usepackage{amsthm}

    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{assumption}{Assumption}
    \newtheorem{conjecture}{Conjecture}
    \newtheorem{proposition}{Proposition}[section]
    \newtheorem{lemma}{Lemma}[section]
    \newtheorem{corollary}{Corollary}[section]
    \newtheorem{algorithm}{Algorithm}[section]
    \newtheorem{definition}{Definition}
    \newtheorem{example}{Example}[section]
    \theoremstyle{definition}
    \newtheorem{remark}{Remark}

 \renewenvironment{proof}[1][Proof]{\noindent \textbf{#1.} }{\  \rule{0.5em}{0.5em}}

%Macro for wrapping text in underbrace
\usepackage{ragged2e}
\newlength\ubwidth
\newcommand\wrapunderbrace[2]{\settowidth\ubwidth{$#1$}\underbrace{#1}_{\parbox{\ubwidth}{\scriptsize\RaggedRight#2}}}


%Allow numbering of one line in align*
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\let\oldemptyset\emptyset
\let\emptyset\varnothing

\providecommand{\keywords}[1]
{
  \small
  \textbf{Keywords:} #1
}

\usepackage[bottom]{footmisc}
\usepackage{xfrac}
\usepackage{bigints}
\allowdisplaybreaks
\emergencystretch 2em
%\renewcommand\arraystretch{1.1}

\expandafter\def\expandafter\normalsize\expandafter{%
    \normalsize%
    \setlength\abovedisplayskip{4pt}%
    \setlength\belowdisplayskip{4pt}%
    \setlength\abovedisplayshortskip{4pt}%
    \setlength\belowdisplayshortskip{4pt}%
}

==> Preambles/notation.tex <==
% Probability
	\renewcommand{\P}{\mathop{}\!\textnormal{P}}
	\newcommand{\E}{\mathop{}\!\textnormal{E}}
	\newcommand{\sE}{\mathop{}\!\mathbb{E}}
	\newcommand{\Cov}{\mathop{}\!\textnormal{Cov}}
	\newcommand{\sCov}{\mathop{}\!\mathbb{C}\textnormal{ov}}
	\newcommand{\Var}{\mathop{}\!\textnormal{Var}}
	\newcommand{\sVar}{\mathop{}\!\mathbb{V}\textnormal{ar}}
	\newcommand{\N}{\mathcal{N}}
	\newcommand{\sN}{\N(0,1)}
	
	\newcommand{\bracks}[1]{\left[#1\right]}
	\newcommand{\expe}[1]{\mathbb{E}\bracks{#1}}
	\newcommand{\expestar}[1]{\mathbb{E}^*\bracks{#1}}
	\newcommand{\expesub}[2]{\mathbb{E}_{#1}\bracks{#2}}
	
	\newcommand{\var}[1]{\mathbb{V}\text{ar}\bracks{#1}}
	\newcommand{\parens}[1]{\left(#1\right)}
    \newcommand{\squared}[1]{\parens{#1}^2}
    \newcommand{\tothepow}[2]{\parens{#1}^{#2}}
    \newcommand{\prob}[1]{\mathbb{P}\parens{#1}}
    \newcommand{\probsub}[2]{\mathbb{P}_{#1}\parens{#2}}

% Convergence
	\newcommand{\Oh}{\mathop{}\!\mathcal{O}}
	\newcommand{\oh}{\mathop{}\!{o}}
	\newcommand{\convd}{\stackrel{d}{\longrightarrow}}
	\newcommand{\convp}{\stackrel{p}{\longrightarrow}}
	\newcommand{\conv}{\stackrel{}{\longrightarrow}}
	
% Basic matrices and vectors
	\newcommand{\0}{\mathbf{0}}
	\newcommand{\1}{\mathbf{1}}
	\newcommand{\I}{\mathbb{I}}
	\renewcommand{\O}{\mathbb{O}}

% Basic maths
	\newcommand{\R}{\mathbb{R}}
	\DeclareMathOperator*{\argmin}{arg\,min}
	\DeclareMathOperator*{\argmax}{arg\,max}
	\newcommand{\Ind}{\mathbbm{1}}  % Indicator
	\newcommand{\reals}{\mathbb{R}}
% Estimation specifics
    \newcommand{\Ih}{\widehat{I}}
    \newcommand{\Is}{\mathcal{I}}
    
% Independence
    \newcommand{\orth}{\perp}
    \renewcommand{\given}{\: | \:}
    
% Prediction
	\newcommand{\X}{\mathcal{X}}  % Covariate space
	\newcommand{\W}{\mathcal{W}}  % Transformed covariate space
	\newcommand{\Y}{\mathcal{Y}}  % Outcome space
	\newcommand{\err}{\varepsilon}  % Outcome error
	\newcommand{\g}{g}  % Truth (conditional expectation/optimal predictor)
	\newcommand{\F}{\mathcal{F}}  % Function class
	\renewcommand{\S}{\ensuremath{S}}  % Sample
	\newcommand{\T}{\ensuremath{T}}  % Training sample
	\renewcommand{\H}{\ensuremath{H}}  % Hold-out sample
	\newcommand{\f}{f}  % Prediction function
	\newcommand{\fh}{\ensuremath{\widehat{f}}}  % Empirical prediction
	\newcommand{\yhat}{\ensuremath{\widehat{y}}}	
	\newcommand{\betahat}{\ensuremath{\widehat{\beta}}}
	\newcommand{\betatilde}{\ensuremath{\tilde{\beta}}}
	\newcommand{\deltatilde}{\ensuremath{\tilde{\delta}}}
	\newcommand{\xtilde}{\ensuremath{\tilde{x}}}
	\newcommand{\Xtilde}{\ensuremath{\tilde{X}}}

	\newcommand{\al}{\ensuremath{\mathcal{L}}}
	\newcommand{\OLS}{\textnormal{OLS}}  % Sendhil does not know how to spell this
	\newcommand{\lh}{\widehat{\lambda}}
    \newcommand{\Z}{\mathcal{Z}}
    \renewcommand{\th}{\widehat{\theta}}
	\newcommand{\Sigmahat}{\ensuremath{\widehat{\Sigma}}}
	\newcommand{\sigmahat}{\ensuremath{\widehat{\sigma}}}
	
%Distributions
\newcommand{\logistic}[2]{\mathrm{Logistic}\parens{#1,\,#2}}
\newcommand{\bernoulli}[1]{\mathrm{Bernoulli}\parens{#1}}
\newcommand{\betanot}[2]{\mathrm{Beta}\parens{#1,\,#2}}
\newcommand{\stdbetanot}{\betanot{\alpha}{\beta}}
\newcommand{\multnormnot}[3]{\mathcal{N}_{#1}\parens{#2,\,#3}}
\newcommand{\normnot}[2]{\mathcal{N}\parens{#1,\,#2}}
\newcommand{\classicnormnot}{\normnot{\mu}{\sigsq}}
\newcommand{\stdnormnot}{\normnot{0}{1}}
\newcommand{\uniform}[2]{\mathrm{U}\parens{#1,\,#2}}
\newcommand{\stduniform}{\uniform{0}{1}}
\newcommand{\exponential}[1]{\mathrm{Exp}\parens{#1}}
\newcommand{\stdexponential}{\mathrm{Exp}\parens{1}}
\newcommand{\gammadist}[2]{\mathrm{Gamma}\parens{#1, #2}}
\newcommand{\poisson}[1]{\mathrm{Poisson}\parens{#1}}
\newcommand{\geometric}[1]{\mathrm{Geometric}\parens{#1}}
\newcommand{\binomial}[2]{\mathrm{Binomial}\parens{#1,\,#2}}
\newcommand{\rayleigh}[1]{\mathrm{Rayleigh}\parens{#1}}
\newcommand{\multinomial}[2]{\mathrm{Multinomial}\parens{#1,\,#2}}
\newcommand{\gammanot}[2]{\mathrm{Gamma}\parens{#1,\,#2}}
\newcommand{\cauchynot}[2]{\text{Cauchy}\parens{#1,\,#2}}
\newcommand{\invchisqnot}[1]{\text{Inv}\chisq{#1}}
\newcommand{\invscaledchisqnot}[2]{\text{ScaledInv}\ncchisq{#1}{#2}}
\newcommand{\invgammanot}[2]{\text{InvGamma}\parens{#1,\,#2}}
\newcommand{\chisq}[1]{\chi^2_{#1}}
\newcommand{\ncchisq}[2]{\chi^2_{#1}\parens{#2}}
\newcommand{\ncF}[3]{F_{#1,#2}\parens{#3}}
\newcommand{\Fnot}[2]{F\parens{#1, #2}}



%shortcuts for Linear Algebra stuff (i.e. vectors and matrices)
\newcommand{\twovec}[2]{\parens{\begin{array}{c} #1 \\ #2 \end{array}}}
\newcommand{\threevec}[3]{\parens{\begin{array}{c} #1 \\ #2 \\ #3 \end{array}}}
\newcommand{\fivevec}[5]{\parens{\begin{array}{c} #1 \\ #2 \\ #3 \\ #4 \\ #5 \end{array}}}
\newcommand{\twobytwomat}[4]{\parens{\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array}}}
\newcommand{\threebytwomat}[6]{\parens{\begin{array}{cc} #1 & #2 \\ #3 & #4 \\ #5 & #6 \end{array}}}
\newcommand{\fourvec}[4]{\parens{\begin{array}{c} #1 \\ #2 \\ #3 \\ #4\end{array}}}
\newcommand{\threebythreemat}[9]{\parens{\begin{array}{ccc} #1 & #2 & #3 \\  #4 & #5 & #6 \\ #7 & #8 & #9 \end{array}}}

%Sign
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\sign}{sign}

% Project specific notation
\newcommand{\betahatpost}{\betahat_{post}}
\newcommand{\betahatpostTN}{\betahat_{post}^{TN}}
\newcommand{\betahatpre}{\betahat_{pre}}
\newcommand{\betatildepost}{\betatilde_{post}}
\newcommand{\betatildepre}{\betatilde_{pre}}
\newcommand{\betapost}{\beta_{post}}
\newcommand{\gammapost}{\gamma_{post}}
\newcommand{\gammahat}{\widehat{\gamma}}
\newcommand{\gammaopt}{\gamma_{*}}
\newcommand{\gammaoptsub}[1]{\gamma_{*#1}}

\newcommand{\gammabar}{\bar{\gamma}}
\newcommand{\gammahatpost}{\widehat{\gamma}_{post}}
\newcommand{\gammahatpostTN}{\widehat{\gamma}_{post}^{TN}}
\newcommand{\gammatilde}{\ensuremath{\tilde{\gamma}}}

\newcommand{\etahat}{\widehat{\eta}}

\newcommand{\deltahat}{\widehat{\delta}}
\newcommand{\deltahatpost}{\deltahat_{post}}
\newcommand{\deltahatpre}{\deltahat_{pre}}
\newcommand{\deltapost}{\delta_{post}}
\newcommand{\deltapre}{\delta_{pre}}

\newcommand{\taupost}{\tau_{post}}
\newcommand{\taupre}{\tau_{pre}}
\newcommand{\taubarone}{\bar{\tau}_1}

\newcommand{\thetabar}{\bar{\theta}}

\newcommand{\Sigmapre}{\Sigma_{pre}}
\newcommand{\Xpre}{X_{pre}}


\newcommand{\CITNbeta}{CI^{TN}_{\beta}}
\newcommand{\CITNgamma}{CI^{TN}_{\gamma}}
\newcommand{\CITrad}{CI^{Trad}}
\newcommand{\betapre}{\beta_{pre}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\xt}{x^t}

\newcommand{\boldy}{\boldsymbol{y}}
\newcommand{\boldytilde}{\boldsymbol{\tilde{y}}}
\newcommand{\boldx}{\boldsymbol{x}}
\newcommand{\boldalpha}{\boldsymbol{\alpha}}
\newcommand{\boldbeta}{\boldsymbol{\beta}}

%\newcommand{\prob}[1]{P\left( #1 \right)}

\newcommand{\tildegammaone}{\tilde{\gamma}_1}
\newcommand{\tildegammamain}{\tilde{\gamma}_{main}}

\newcommand{\taubar}{\bar{\tau}}
\newcommand{\tautilde}{\tilde{\tau}}
\newcommand{\tildetau}{\tautilde}


%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\ubar}[1]{\underline{$#1$}}

\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

\newcommand{\Tau}{\mathrm{T}}

\newcommand{\Bcal}{\mathcal{B}}

\newcommand{\Atilde}{\tilde{A}} 
\newcommand{\Atildeone}{\tilde{A}_{(\cdot,1)}} 
\newcommand{\Atildeminus}{\tilde{A}_{(\cdot,-1)}} 
\newcommand{\Atildebone}{\Atilde_{(B,1)}}
\newcommand{\Atildeminusbone}{\Atilde_{(-B,1)}}
\newcommand{\Atildebminus}{\Atilde_{(B,-1)}}
\newcommand{\Atildeminusbminus}{\Atilde_{(-B,1)}}

\newcommand{\sigmatilde}{\tilde{\sigma}}
\newcommand{\Sigmatilde}{\tilde{\Sigma}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\mutilde}{\tilde{\mu}}
\newcommand{\alphatilde}{ \tilde{\alpha} }
\newcommand{\deltatildepre}{ \tilde{\delta}_{pre} }
\newcommand{\deltatildepost}{ \tilde{\delta}_{post} }

\newcommand{\deltabar}{ \bar{\delta} }
\newcommand{\deltabarpre}{ \bar{\delta}_{pre} }
\newcommand{\Deltapre}{\Delta_{pre}}

\newcommand{\mubar}{\bar{\mu}}
\newcommand{\Yhat}{\widehat{Y}}

% Tests and CIs
\newcommand{\condtest}[1]{\psi^{C}_{#1}}
\newcommand{\condci}{\mathcal{C}^{C}_{\alpha, n}}
\newcommand{\condteststar}{\psi^{C}_{*, \alpha}}

\newcommand{\MPtest}[1]{\psi^{MP}_{#1}}
\newcommand{\LFtestcustomalpha}[1]{\psi^{LF}_{#1}}

\newcommand{\condLFtest}{\psi^{C \mhyphen LF}_{\kappa, \alpha}}
\newcommand{\condLFteststar}{\psi^{C \mhyphen LF}_{*, \kappa, \alpha}}
\newcommand{\condLFci}{\mathcal{C}^{C \mhyphen LF}_{\kappa, \alpha, n}}

\newcommand{\condFLCItest}{\psi^{C \mhyphen FLCI}_{\kappa,\alpha}}
\newcommand{\condFLCIci}{\mathcal{C}^{C \mhyphen FLCI}_{\kappa, \alpha, n}}

\newcommand{\FLCInon}[1]{\mathcal{C}^{FLCI}_{#1}}
\newcommand{\FLCI}[1]{\mathcal{C}^{FLCI}_{#1, n}}
\newcommand{\LFtest}{\psi^{LF}_{\kappa}}

\newcommand{\scaledv}{v}
\newcommand{\unscaledv}{\breve{v}}
\newcommand{\scaleda}{a}
\newcommand{\unscaleda}{\breve{a}}
\newcommand{\scaledchi}{\chi}
\newcommand{\unscaledchi}{\breve{\chi}}



\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
